Imagined Value Gradients: Model-Based Policy Optimization with Transferable Latent Dynamics Models

Humans are masters at quickly learning many complex tasks, relying on an approximate understanding of the dynamics of their environments. In much the same way, we would like our learning agents to quickly adapt to new tasks. In this paper, we explore how model-based Reinforcement Learning (RL) can facilitate transfer to new tasks. We develop an algorithm that learns an action-conditional, predictive model of expected future observations, rewards and values from which a policy can be derived by following the gradient of the estimated value along imagined trajectories. We show how robust policy optimization can be achieved in robot manipulation tasks even with approximate models that are learned directly from vision and proprioception. We evaluate the efficacy of our approach in a transfer learning scenario, re-using previously learned models on tasks with different reward structures and visual distractors, and show a significant improvement in learning speed compared to strong off-policy baselines. Videos with results can be found at https://sites.google.com/view/ivg-corl19

==> Model Based RL SVGN for Robot Control/approach_final.tex <==
%===============================================================================
\vspace{-0.2cm}
\section{Background}
\vspace{-0.2cm}
%\akb{I have structured this similar to the VPN paper and a lot of the math/MDP background stuff is borrowed from the SVG \& VPN papers. Change it if it is too similar to them.}\\

We are interested in solving motor control problems such as robotic manipulation tasks from vision. 
This setup can be formalized as a partially observed Markov decision process (a POMDP) with observation $\bO^t \in R^{N_O}$, states $\sS^t \in R^{N_S}$, actions $\bA^t \in R^{N_A}$ 
%TOBICOPY The latent state space is constructed via a deterministic mapping from the observations: $\bS^t = f_{\text{enc}}(\bO^{1:t})$ To obtain low-variance estimates in the policy optimization, we will consider systems that can be described with deterministic latent state spaces (although the observations could, in principle, be stochastic realizations). 
transition probabilities $p(\sS^{t+1} | \sS^{t}, \bA^t)$,
%= p(\sS^{t+1} | \bO^{1:t}, \bA^t)$. 
and reward function $r^t = r(\sS^t, \bA^t)$. %This MDP mirrors the ``true environment'' MDP in the observation space $O$: $\bar{\mathcal{M}} = (O, A, \bar{p}, \bar{r})$, sharing the same action space $A$ with the transition probability distribution $\bar{p}(o^{t+1} | o^{1:t}, a^t)$ and reward $\bar{r}$ functions operating on observations $\bO^t$. 
Let $\tau_{\leq t} = (\bO^{1:t}, \bA^{1:t-1})$ be the sequence of observations and actions in a trajectory up to decision point $t$.
The optimal policy and the value function at time step $t$ in this setting are a function of the posterior of the system state $p(\sS_t | \tau_{\leq t})$ given the interaction history. However, this posterior is usually intractable and many reinforcement learning approaches resort, instead, to directly optimizing a parametric policy that is a function of the history $\tau_{\leq t}$, i.e.\ they consider policies of the form $\pi(\bA_t | \tau_{\leq t})$.
Thus, they aim to maximize the sum of discounted rewards: $J(\theta) = \mathbb{E}_{p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})}\left[ \sum_{t=0}^T \gamma^t r^t\right]$, with discount factor $\gamma \in [0, 1)$, where the trajectory distribution is assumed to decompose into transition and action probabilities as 
$
p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t}) = p(\sS^t | \tau_{\leq t}) \prod_{t' \geq t}^{T-1} \pi(\bA^{t'} | \tau_{\leq t'}) p(\sS^{t'+1} | \sS^{t'}, \bA^{t'}) p(\bO^{t'+1} | \sS^{t'+1}).
$
This allows us to define the value of an observed trajectory prefix as 
\begin{equation}
\textstyle
%V^\pi(\sS^t) =
V^\pi(\tau_{\leq t}) = \mathbb{E}_{p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})} \left[ \sum_{k=t}^T \gamma^{k-t} r^t 
%| \sS^t = \sS 
\right],
\label{eqn:true_v}
\end{equation}
where, below, we consider the  infinite horizon case" $\lim_{T \to \infty}$.


% %------
% We consider discrete-time Markov Decision Processes with continuous observations, states and actions -- i.e. the system might be partially observed (a POMDP). Let us denote the observation, a history of observations (with length $t$), state and action at time $t$ by $\bO^t \in R^{N_O}$, $\bO^{1:t} \in R^{t \times N_O}$,  $\sS^t \in R^{N_S}$, $\bA^t \in R^{N_A}$ respectively. 
% %TOBICOPY The latent state space is constructed via a deterministic mapping from the observations: $\bS^t = f_{\text{enc}}(\bO^{1:t})$ To obtain low-variance estimates in the policy optimization, we will consider systems that can be described with deterministic latent state spaces (although the observations could, in principle, be stochastic realizations). 
% The evolution of states over time is described via  transition probabilities $p(\sS^{t+1} | \sS^{t}, \bA^t)$.
% %= p(\sS^{t+1} | \bO^{1:t}, \bA^t)$. 
% the POMDP is completed by a reward function $r^t = r(\sS^t, \bA^t)$. %This MDP mirrors the ``true environment'' MDP in the observation space $O$: $\bar{\mathcal{M}} = (O, A, \bar{p}, \bar{r})$, sharing the same action space $A$ with the transition probability distribution $\bar{p}(o^{t+1} | o^{1:t}, a^t)$ and reward $\bar{r}$ functions operating on observations $\bO^t$. 
% Let $\tau_{\leq t} = (\bO^{1:t}, \bA^{1:t-1})$ be the collection of observations and actions observed in a trajectory up to decision point $t$.
% The optimal policy and the value function at time step $t$ in this setting are a function of the posterior of the system state $p(\sS_t | \tau_{\leq t})$ given the interaction history. However, this posterior is usually intractable and many reinforcement learning approaches resort, instead, to directly optimizing a parametric policy that is a function of the history $\tau_{\leq t}$, i.e.\ they consider policies of the form $\pi(\bA_t | \tau_{\leq t})$.
% Thus, they aim to maximize the sum of discounted rewards: $J(\theta) = \mathbb{E}_{p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})}\left[ \sum_{t=0}^T \gamma^t r^t\right]$, with discount factor $\gamma \in [0, 1)$, where the trajectory distribution is assumed to decompose into transition and action probabilities as 
% $
% p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t}) = p(\sS^t | \tau_{\leq t}) \prod_{t' \geq t}^{T-1} \pi(\bA' | \tau_{\leq t'}) p(\sS^{t'+1} | \sS^{t'}, \bA^{t'}) p(\bO^{t'+1} | \sS^{t'+1}).
% $
% From this, we can also also define the value function of an observed trajectory as 
% \begin{equation}
% %V^\pi(\sS^t) =
% V^\pi(\tau_{\leq t}) = \mathbb{E}_{p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})} \left[ \sum_{k=t}^T \gamma^{k-t} r^t 
% %| \sS^t = \sS 
% \right],
% \label{eqn:true_v}
% \end{equation}
% where, below, we consider the common infinite horizon case; $\lim_{T \to \infty}$.
% %-----

\vspace{-0.2cm}
\section{An Action-Conditional Expectation Model of Observations and Rewards}
\vspace{-0.2cm}

Naively, a model-based evaluation of \eqref{eqn:true_v} would require an accurate action-conditional model of future observations and rewards given a a partial trajectory $\tau_{\leq t}$. Especially in high-dimensional observation spaces such a model can be difficult to learn.
%
%
% We are interested in a model based RL solution for finding $\pi$ in the scenario described above. Unfortunately, modeling the distributions comprising %$p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})$
% $p_\pi(r^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})$
% -- to estimate Equation \eqref{eqn:true_v} for model based RL -- can be difficult  \citep{TODONicolasadd} that as it involves fitting a probabilistic models of all potential future observations, and rewards, given a partial trajectory. 
%
Instead we consider an approximate model suitable for weakly partially observed domains with limited stochasticity. 
%(We discuss model limitations in Sec.~\ref{sec:model:limitations}.) 
We develop a latent state-space model whose latent state at time step $t$ is optimized to represent a sufficient statistic of the interaction history $\tau_{\leq t}$. The model is trained to predict expectations of future observations and reward by approximately modeling the evolution of the summary statistic via a deterministic transition model.
%As a simplification we instead fit a latent state-space model whose latent state at time step $t$ is optimized to represent a sufficient statistic of the interaction history $\tau_{\leq t}$. The model is trained to predict expectations of future observations and reward by approximately modeling the evolution of the summary statistic via a deterministic transition model.
%
%As a simplification we instead fit a latent state-space model whose latent state at time step $t$ is optimized to represent a sufficient statistic of the interaction history $\tau_{\leq t}$. The model is trained to predict expectations of future observations and reward by approximately modeling the evolution of the summary statistic via a deterministic transition model.
%
We express the policy as a function of the latent state and the model allows us to construct a surrogate model $\VM$ that expresses the value $V^\pi(\tau_{\leq t})$ as a recursive function of the policy, the deterministic transition function, and a learned approximation to the reward. This surrogate model can be used to compute approximate policy gradients.
%

More specifically, we let $\bS^t = f_\text{enc}(\bO^{1:t}; \phi)$ be a determistic mapping (with parameters $\phi$) extracting a summary statistic from 
%latent state from 
a history of observations\footnote{We drop the dependency on actions here, assuming $\sS$ is retrievable from a history of observations only.}; and we let $\bS^{t+1} \triangleq f_{\text{trans}}(\bS^t, \bA^t; \phi)$ denote a latent transition function. %As noted above and discussed in more detail below (\ref{XXX}) we make the simplifying assumption that  any expectation of future observations or rewards can be represented as a deterministic function of $\bS^t$ conditioned on future actions. 
The assumption that the latent dynamics are well described by a deterministic transition function is our primary simplification.
We further define the approximate reward function based on latent states as $\rE(\bS^t, \bA^t; \phi) = \rE( f_\text{trans}(\bS^t, \bA^t); \phi)$ which we calculate by chaining the transition model with a reward predictor. Finally, we denote with $\pi_\theta(\bA | \bS)$ a 
stochastic policy, parameterized by $\theta$. Using these definitions we construct an approximation of the expectation in Eq. \eqref{eqn:true_v} as $V^\pi(\tau_{\leq t}) \approx \VM^\pi(\bS^t) = \mathbb{E}_{\pi_\theta} \left[ \sum_{k=t}^\infty \gamma^{k-t} \rE^k | \bS^t = \bS \right]$ or, written recursively:
\begin{equation}
    V^\pi(\tau_{\leq t}) \approx \VM^\pi(\bS^t) = \int \left[ \rE(\bS^t, \bA; \phi) + \gamma \VM^\pi(\bS^{t+1}) \big| \bS^{t+1} = f_{\text{trans}}(\bS^t, \bA; \phi) \right] \pi_{\theta}(\bA | \bS^t) \mathrm{d}\bA,
    \label{eqn:value}
\end{equation}
where the initial latent state is given as $\bS^t = f_{\text{enc}}(\bO^{1:t}; \phi)$.
%where we have used the fact that the transition dynamics is assumed to be deterministic, i.e.: $\bSp \triangleq \bS^{t+1} = f_{\text{trans}}(\bS, \bA)$. 
In the following we will describe our approach in two steps: We first describe how to learn the action-conditional model for $f_\text{enc}, f_\text{trans}$, $\rE$, and thus $\VM$ in Sec.~\ref{sec:model}. We then explain in Sec.~\ref{sec:policylearn} how the model can be used to optimize the policy. %We conclude with a discussion of the model's limitations (Section \ref{sec:model:limitations}).

\vspace{-0.2cm}
\subsection{Model Learning} \label{sec:model}
We need to estimate all quantities comprising Equation \eqref{eqn:value}; i.e., we need to estimate the following parametric functions (for brevity we use a single set of parameters $\phi$ for all model parameters):
\begin{center}
\begin{tabular}{ l l }
\textbf{Encode }$f_{enc}(\bO^{1:t}; \phi) = \bS^t \approx \mathbb{E}_{p(\sS | \bO^{1:t})}[\sS^t]$ &
\textbf{Transition }$f_{trans}(\bS^t, \bA; \phi) = \bS^{t+1}$ \\
\textbf{Decode }$f_{dec}(\bS^t; \phi) \approx \mathbb{E}_{p(\bO | \sS^t, \tau_{\leq t})}[\bO^t]$ &
\textbf{Value} $\VE^{\pi}(\bS^t; \phi) \approx V^\pi(\tau_{\leq t})$ \\
\multicolumn{2}{l}{\textbf{Reward} $\rE(\bS^t, \bA^t; \phi) = \rE(f_\text{trans}(\bS^t, \bA^t); \phi) \approx
\mathbb{E}_{p(\sS^t |  \tau_{\leq t}, \bA^t)}
[r(\sS^t, \bA^t)]$}
\end{tabular}
\end{center}
The \textbf{Encoder} maps a history of observations $\bO^{1:t}$ to a summary statistic or latent state $\bS^t$, via a recurrent neural network. 
%to learn the deterministic mapping into an \textit{abstract, unstructured latent representation}. 
Recurrence allows us to handle partially observable settings (eg: occlusion). 
The \textbf{Transition} function predicts the next latent state $\bS^{t+1}$ given the current state $\bS^t$ and action $\bA$, evolving dynamics in the low-dimensional latent space. %%We use a feed-forward fully-connected neural network as our transition model.
The \textbf{Decoder} maps the latent $\bS^t$ back to an expected observation $\bO^t$ and is primarily used as self-supervision for training the encoder \citep{wayne2018unsupervised}. %The decoder uses a de-convolutional architecture to reconstruct the images from latent state and fully-connected layers to predict the proprioception output.
The \textbf{Value} function, predicts the sum of expected rewards (the value) as a function of a latent $\bS^t$.
Lastly, the \textbf{Reward} function predicts the immediate, expected reward for a given latent state-action pair. Please refer to Section E of the supplementary for additional details on the model architecture. %Additional details on the architecture of the model components and a schematic of an $N$-step rollout through the model are provided in the supplementary. %(Sec.~\ref{sec:modelarch}).

%\item The \textbf{Policy} module learns the mapping from latent state to actions, predicting a distribution from which we can sample actions.
%To approximate Equation \eqref{eqn:value} -- and its gradient --  using these functions, we will have to define a loss based on trajectories acquired by interacting with the environment.
For the model-based value function $\VM$ in Eq.~\eqref{eqn:value} to form a good approximation of the true value $V^\pi$ (and its gradient) we train the model on trajectories collected while interacting with the environment.
%Assume, for now, that we have available a buffer $\mathcal{B}$ of such trajectory data, under an arbitrary behavior policy $\mu(\bA | \bS)$. 
The main approximation of our approach is the assumption that the evolution of the latent state is well modeled by a deterministic transition function. In partially observed and stochastic environments this is not guaranteed. For the relevant quantities to be well approximated despite this simplification we employ a number of losses that satisfy the following desiderata:
i) we want to ensure that $\bS^t$ is a sufficient statistic of the history $\bO^{1:t}$ and the system thus Markov in $\bS$; ii) we want to minimize the discrepancy between the predicted and observed evolution of the latent state $\bS$;
iii) given a latent state $\bS^t$ we want to accurately predict the expected reward and value (of policy $\pi$) at time step $t+k$ after executing some action sequence $\bA^{t:t+k}$.
%that we expect to obtain when executing policy $\pi$;
%iv) we want to minimize the discrepancy between our approximate value $\VE^\pi(\bS^t)$ and the true value $V^\pi(\sS^t)$.
%, this amounts to regressing rewards and values (for bootstrapping) from predicted latent states (c.f. $\mathcal{L}_r$, $\mathcal{L}_V$).
%The goal of learning is concisely described by two desiderata: 
%i) we want to ensure that latent state trajectories capture the expected dynamics of the true environment (see $L_f$ below) ii) we want to minimize the discrepancy between our approximate value $V^\pi(\bS^t)$ and the true value $V^\pi(\sS^t)$, this amounts to regressing rewards and values (for bootstrapping) from predicted latent states (c.f. $\mathcal{L}_r$, $\mathcal{L}_V$).
%

Let $\mathcal{B}$ denote a set of trajectory data collected while executing some behavior policy $\mu(\bA | \bS)$.
Let us define the full model loss after an initial ``burn-in'' of $H$ steps (to ensure the encoder has sufficient information) as $ \mathcal{L}^N = \mathbb{E}_{p_\pi,\mu} [ \sum_{t=H+1}^{H+N-1}  \mathcal{L}_e(\bS^t, \bA^t, r^{t}, \bO^{1:t+1}) |f_\text{trans}, f_{\text{enc}} ]$ where we approximate the expectation wrt. %$p_\pi(\sS^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})$ 
$p_\pi(r^{t:T}, \bA^{t:T}, \bO^{t+1:T} | \tau_{\leq t})$ 
with samples from $\mathcal{B}$,
\begin{equation}
%\begin{aligned}
    \mathcal{L^N} \approx \mathbb{E}_{\tau \sim \mathcal{B}} \left[ \sum_{t=H+1}^{H+N-1}  \mathcal{L}_e(\bS^t, \bA^t, r^{t}, \bO^{1:t+1}) \Big| \bS^{t+1} = f_\text{trans}(\bS^t, \bA^t; \phi), \bS^{H} = f_{\text{enc}}(\bO^{1:H}; \phi) \right],
    %\mathcal{L}^N = \mathbb{E}_{p_\pi,\mu} &\left[ \sum_{t=H+1}^{H+N} \mathcal{L}_f(\bS^t, \bO^{1:t}) + \alpha \mathcal{L}_{r}(\bS^t, 
    %\bA^t, r^t) + \beta \mathcal{L}_{V}(\bS^t, \bA^t, r^{t}, \bS^{t+1}) \Big| f_\text{trans}, f_{\text{enc}} \right] \\
    %\approx \mathbb{E}_{(\bO^{1:N}, \bA^{1:N}, r^{1:N}) \sim \mathcal{B}} &\left[
    %\sum_{t=H+1}^{H+N} \mathcal{L}_f(\bS^t, \bO^{1:t}) + \alpha \mathcal{L}_{r}(\bS^t, 
    %\bA^t, r^t) + \beta \mathcal{L}_{V}(\bS^t, \bA^t, r^{t}, \bS^{t+1}) \Big| f_\text{trans}, f_{\text{enc}} \right],
%\end{aligned} 
\label{eqn:modelloss}
\end{equation}
with $\tau := (\bO^{1:H+N}, \bA^{1:H+N}, r^{1:H+N})$ and where the per example loss is defined as $\mathcal{L}_e = \mathcal{L}_f(\bS^t, \bO^{1:t}) + \alpha \mathcal{L}_{r}(\bS^t, \bA^t, r^t) + \beta \mathcal{L}_{V}(\bS^t, \bA^t, r^{t}, \bO^{1:t+1})$. $\alpha$ and $\beta$ are %loss multipliers
coefficients that 
%defining 
determine the relative contribution of the loss components. The per example transition model loss is given as
\begin{equation}
\begin{aligned}
\mathcal{L}_f(\bS^t, \bO^{1:t}) = \| f_{\text{dec}}(\bS^t; \phi) - \bO^t \|_2^2 + \zeta \|f_{\text{enc}}(\bO^{1:t}; \phi) - \bS^t \|_2^2,
\end{aligned}
\end{equation}
where the first term measures the error between the observations $\bO$ and reconstructions from the open-loop latent state predictions ($\bS^{t>H}$) and the second term
enforces consistency between the latent state representation from the encoder $f_{\text{enc}}$ and the predictions from the transition model $f_\text{trans}$; this encourages the latent state to stay close to encodings of observed trajectories thus addressing points i) and ii) above. Here $\zeta$ is a coefficient that weights the two loss terms and the reward loss is 
\begin{equation}
\begin{aligned}
\mathcal{L}_{r}(\bS^t, \bA^t, r^t) = \| \rE(\bS^t, \bA^t; \phi) - r^t \|_2^2,
\end{aligned}
\end{equation}
where the value-loss is given by the, importance weighted, squared Bellman error 
\begin{equation}
\begin{aligned}
\mathcal{L}_{V}(\bS^t, \bA^t, r^{t}, \bO^{1:t+1}) = \frac{\pi(\bA^t | \bS^t)}{\mu(\bA^t | \bS^t)} \left(r^t + \gamma \VE^\pi(f_\text{enc}(\bO^{1:t+1}; \psi); \psi) - \VE^\pi(\bS^t; \phi)\right)^2,
\end{aligned}
\label{eqn:value_loss}
\end{equation}
where the next state value $\VE^\pi(f_\text{enc}(\bO^{1:t+1}; \psi); \psi)$ is calculated via a ``target network'', whose parameters $\psi$ are periodically copied from $\phi$, to stabilize training (see e.g. \cite{mnih2015human} for a discussion). In practice we use a v-trace target~\citep{espeholt2018impala}; see discussion in the supplementary. Note that both loss terms are evaluated for \emph{predicted} latent states with gradients flowing backwards through the transition model and eventually the encoder, which addresses point iii). We encourage the reader to consult to Section C \& Figure 1 in the supplementary material for additional details and a schematic.

% \begin{figure}
%     \centering
%     \resizebox{12cm}{!}{\input{figures/modelrollout.tex}}
%     \caption{\textit{Left}: Graph showing the rollout of a sequence of observations and actions $\tau$ (red circles), through the model (gray rectangles), predicting latent states and their corresponding reconstructed observations (blue circles). There are two stages: 1) Encoding the observations to the latent space (green block), followed by 2) an open loop rollout in the latent space, starting from the latent state $\bS^H$ (after a burn-in of length $H$) and applying the sequence of actions $\bA^{H:H+N-1}$ (yellow block). \textit{Right}: Actor execution of the policy. The past $H$ observations are encoded to generate state $\bS^t$ which is fed to the policy to generate action $\bA^t$.}
%     \label{fig:modelactorrollout}
% \end{figure}

% \subsection{Limitations}
% \label{sec:model:limitations}
% The main approximation in our modeling approach is the assumption that the evolution of the latent state is well modeled by a deterministic transition function. In partially observed and stochastic environments this is not guaranteed. However, the losses described in Section \ref{sec:model} are designed to ensure that the relevant quantities will be well approximated despite this simplification.

\vspace{-0.2cm}
\section{Imagined Value Gradients in Latent Spaces}
\vspace{-0.2cm}
\label{sec:policylearn}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/training/policytraining.pdf}
    \caption{Imagined policy gradient computation. Given a history $H$ of observations from $\mathcal{B}$, we encode a latent state $\bS^H$, followed by an ``imagined'' rollout of length $N$ -- using sequence of sampled actions $\bA^{t>H}$ and $f_{trans}$. This leads to imagined states $\bS^{t>H}$ with corresponding value and reward estimates. We average cumulative rewards over $N$ horizons -- computing the estimate from Eq.~\eqref{eqn:svgn_avg_full}.}
    \label{fig:imaginedrollout}
    \vspace{-0.4cm}
\end{figure}

Given a model, we optimize a parametric policy $\pi_\theta(\bA | \bS)$ by maximizing the N-step surrogate value function which is a recursive composition of the policy, the transition, reward and value function:
\begin{equation}
    \VM_N(\bS^t) = \mathbb{E}_{\bA^k \sim \pi} \left[ \gamma^{N} \VE^\pi(\bS^{t+N}; \phi) + \sum_{k=t}^{t+N-1} \gamma^{k-t} \rE(\bS^k, \bA^k) \Big| \bS^{k+1} = f_\text{trans}(\bS^k, \bA^k) \right],
    \label{eqn:value_n}
\end{equation}
This N-step value can be computed by performing an ``imagined'' rollout in the latent state-space using our model (see ~\figref{fig:imaginedrollout}).
It can be maximized by gradient ascent, exploiting the so called ``value gradient''  $\nabla_\theta{\VM}_N(\bS^t)$ \citep{heess2015learning}; which can often be computed recursively, taking advantage of the reparameterization trick \citep{kingma2013auto,rezende2014stochastic} for sampling from $\pi_\theta$ and calculating analytic gradients via backpropagation backwards through time. We can express the policy as a deterministic function $\pi_\theta(\bS^t, \epsilon)$ that transforms a sample $\epsilon$ from a canonical noise distribution $p(\epsilon)$ into a sample from $\pi_\theta(\bA | \bS)$. In the following we will consider Gaussian policy distributions, i.e. $\pi_\theta(\bA | \bS) = \mathcal{N}(\mu_\theta(\bS), \sigma^2_\theta(\bS))$, for which the reparameterization is given as $\pi_\theta(\bS, \epsilon) = \mu_\theta(\bS) + \epsilon \sigma_\theta(\bS)$, with $p(\epsilon) = \mathcal{N}(\mathbf{0}, \mathbf{I})$, where $\mathbf{I}$ denotes the identity matrix. We can then calculate the gradient $\nabla_\theta\VM_N(\bS^t)$ for any state as
% \begin{equation}
%  \nabla_\theta{\VM}_{N}(\bS^t) = \! \! \!\!\! \sum_{k=t}^{t+N-1} \!\!\mathbb{E}_{p(\epsilon)} \Big[  \nabla_\theta \rE(\bS^{k}, \pi_\theta\big(\bS^{k}, \epsilon)\big) + \gamma \nabla_{\bS^{k+1}} {\VM}_{N-k}(\bS^{k+1}) \nabla_\theta f_\text{trans}\big(\bS^{k}, \pi_\theta(\bS^{k}, \epsilon)\big) \Big],
% \label{eqn:svgn_theta}
% \end{equation}
% \begin{equation}
% \nabla_\theta{\VM}_N(\bS^t) = \mathbb{E}_{p(\epsilon)} \big[\nabla_\theta \rE\big(\bS^{t}, \pi_\theta(\bS^{t}, \epsilon)\big) + \gamma \nabla_{\bS^{t+1}} \VM_{N-1}(\bS^{t+1}) \nabla_\theta f_\text{trans}\big(\bS^{t}, \pi_\theta(\bS^{t}, \epsilon)\big) + \gamma \nabla_\theta{\VM}_{N-1}(\bS^{t+1}) \big]
% \label{eqn:svgn_theta}
% \end{equation}
%\begin{equation}
%\nabla_\theta{\VM}_N(\bS^t) = \mathbb{E}_{p(\epsilon)} \big[\nabla_\theta \rE\big(\bS^{t}, \pi_\theta(\bS^{t}, \epsilon)\big) + \gamma \nabla_{\bS^\prime} \VM_{N-1}(\bS^\prime) \nabla_\theta f_\text{trans}\big(\bS^{t}, \pi_\theta(\bS^{t}, \epsilon)\big) + \gamma \nabla_\theta{\VM}_{N-1}(\bS^\prime) \big]
%\label{eqn:svgn_theta}
%\end{equation}
\begin{equation}
\nabla_\theta{\VM}_N(\bS^t)\!\! = \!\!\mathbb{E}_{p(\epsilon)} \big[\big(\nabla_\bA \rE\big(\bS^{t}, \bA\big)\! +\! \gamma \nabla_{\bS^\prime} \VM_{N-1}(\bS^\prime) \nabla_\bA f_\text{trans}\big(\bS^{t}, \bA\big)\big) \nabla_\theta \pi_\theta(\bS^{t}, \epsilon)\! + \! \gamma \nabla_\theta{\VM}_{N-1}(\bS^\prime) \big]
\label{eqn:svgn_theta}
\end{equation}
where $\bS^\prime := \bS^{t+1} = f_\text{trans}(\bS^{t}, \pi_\theta(\bS^{t}, \epsilon))$ and we dropped the dependencies on $\phi$ for brevity. The value gradient $\nabla_{\bS^\prime} {\VM}_{N-1}(\bS^\prime)$ wrt. a state $\bS^\prime$ is defined recursively and provided in Eq.~(3) in the supplementary material.
The case $\nabla_\theta{\VM}_{1}(\bS^{t+N})$ is established by assuming the policy is fixed in all steps after $N$; i.e. bootstrapping with $\nabla_{\bS^{t}}\VM_0(\bS^{t}) = \nabla_{\bS^{t}}\VE^\pi(\bS^{t}; \phi)$. To calculate the gradient, only an initial state $\bS^t$ (encoded from $\bO^{1:t} \sim \mathcal{B}$) is required (see \figref{fig:imaginedrollout}). Eq.\ \eqref{eqn:svgn_theta} computes $N$ policy gradient contributions for the encoded state $\bS^t$ as well as for the imagined states $\bS^{t+1} \dots \bS^{t+N-1}$. This ensures that the policy can be evaluated on either kind of latent state. Our derivation is analogous to SVG \citep{heess2015learning}; but using imagined latent states and assuming a deterministic transition model.


%Talk about policy, value \& reward functions. Then given a sequence of observations, actions \& rewards we discuss how to train the entire system together (including the model).


%Model uses the rollout and losses from above. Reward uses the true reward basically (from trans model states?). Value uses target networks + retrace but we predict values from model rollouts and compare it to target network predictions on true encoded states or the model rollouts. Which? Write out whole loss and mention that model is trained jointly and all losses here backprop to model so that representation is good for predicting value \& reward. We can discuss fitted value learning etc in supplementary.


%Using sequence of observations, actions and rewards. Show how the rollout works, write out the math for the value function learning, write out the losses for the model \& reward network, mention that these parameters share gradients so model gets gradients from reward, value, decoder etc. Add a fitted value learning algorithm similar to the SVG paper in supplementary. Mention that thsi part is pretty much same as SVG but with Retrace \& latent representation learning. Talk about burn-in / history with the recurrent model.

\vspace{-0.2cm}
\subsection{Stable Regularized Policy Optimization}
We make the following observations regarding the use of value gradients in practice:
%We make a few interesting observations relevant to the value gradients use in practice. 
First, we can obtain different gradient estimators by varying $N$. For small $N$ we obtain a more biased value gradient -- due to the reliance on bootstrapping -- that changes slowly (i.e. it changes at the speed of convergence for $\VE^\pi(\bS; \phi)$). For large $N$, less bias, and faster learning could be achieved if model and reward predictors are accurate, but the estimate can be affected by modelling errors. As a compromise, we found that averaging gradient estimates obtained with different-length rollouts worked well in practice
$
    \nabla_\theta{\bar{V}}_N(\bS) = \frac{1}{N} \sum_{k}^N \nabla_\theta{\VM}_k(\bS).
    \label{eqn:svgn_avg}
$
We refer to the supplementary for details.

Second, even with this averaged gradient, optimization is prone to exploiting modelling errors (in the transition dynamics and reward/value estimates) -- see e.g. \citep{planet-dm} for a discussion. To counteract this, we employ relative-entropy (KL) regularization. Similar to existing policy optimization methods \citep{schulman2017proximal,abdolmaleki2018maximum,haarnoja2018soft} we augment the estimated reward with a KL penalty, yielding
$
    \rE_\text{KL}(\bS, \bA, \pi_\theta) = \rE(\bS, \bA) + \lambda \log\frac{\pi_\theta(\bA | \bS)}{p(\bA | \bS)},
$
where $p(\bA | \bS)$ is a the prior action probability (we use $p(\bA | \bS) = \mathcal{N}(\mathbf{0}, \mathbf{I})$ throughout) and $\lambda$ is a cost multiplier. Replacing $\rE$ in Equation \eqref{eqn:svgn_theta} with $\rE_\text{KL}$ -- noting that $\rE_\text{KL}$ is differentiable wrt. $\theta$ -- results in the regularized value gradient $\nabla_\theta{\VM}^{\text{KL}}_{N}(\bS)$.
Analogously, we obtain a compatible value ${\VM}^{\text{KL}}_{0}(\bS)$ by replacing $r$ with $r_\text{KL}$ in Equation \eqref{eqn:value_loss}. The total derivative estimate we use then is
\begin{equation}
\textstyle
       \nabla_\theta \mathbb{E}_{p_{\pi}} \Big[ \bar{V}^{\text{KL}}_N(\bS^t) \Big] \approx \mathbb{E}_{\bO^{1:t} \sim \mathcal{B}} \Big[ \frac{1}{N} \sum_{k=1}^N \nabla_\theta{\VM}^\text{KL}_k(f_\text{enc}(\bO^{1:t})) \Big],
    \label{eqn:svgn_avg_full}
\end{equation}
where we use batches from the replay to optimize the policy on all visited states -- using Eq.~\eqref{eqn:svgn_avg_full} in combination with Adam \cite{kingma2014adam}. 
%The full learning procedure involves executing the most recent policy to populate the replay buffer $\mathcal{B}$ in parallel with model and policy optimization using the model loss from Eq.~\eqref{eqn:modelloss} and the averaged policy gradient from Eq.~\eqref{eqn:svgn_avg_full}. 
Please refer to Algorithm (1) in the supplementary for a  description.

%by minimizing the model loss from Eq.~\eqref{eqn:modelloss} and maximizing the value estimate via the averaged policy gradient from Eq.~\eqref{eqn:svgn_avg_full} respectively. Please refer to Algorithm~\ref{alg:overall} in the supplementary for a full description.

%is also described in Algorithm.~\ref{alg:overall}. %\akb{this is a simple algorithm that references the eqns above}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}[t]
% \caption{Imagined Value Gradients in Latent Spaces}
% \label{alg:overall}
% %\small
% \begin{algorithmic} 
% \STATE {Given: Empty experience dataset $\mathcal{B}$, burn-in $H$, rollout length $N$, episode length $T$}
% \STATE \textbf{Each actor do:}
%     \bindent
%     %%%%%% Actor loop
%     \WHILE{True}
%     \STATE Fetch policy / model parameters ($\theta$, $\phi$) from learner; Initialize empty trajectory $\tau:=\emptyset$
%     \FOR{t = 0 to T} 
%     \STATE Apply control $\pi_{\theta}(f_{enc}(\bO^{t-H:t}; \phi), \epsilon), \ \epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ \COMMENT{Encode history, take action}
%     \STATE Observe $r,\bO^\prime$; Insert ($\bO, \bA, r, \bO^\prime$) into $\tau$  
%     \ENDFOR
%     \STATE Save $\tau$ in the dataset $\mathcal{B}$
%     \ENDWHILE
%     \eindent

% \STATE \textbf{Learner do:}
%     \bindent
%     \WHILE{True}
%     %%%%%% Learner loop
%     \STATE Sample sub-trajectory of length $H+N$ from buffer: $(\bO^{1:H+N}, \bA^{1:H+N}, r^{1:H+N}) \sim \mathcal{B}$
%     \STATE Compute $\nabla_{\phi} \mathcal{L}^{\mathcal{N}}$, the gradient of Eq.~\ref{eqn:modelloss} w.r.t model, reward and value parameters $\phi$
%     \STATE Compute the policy gradient $\nabla_\theta \mathbb{E}_{p_\pi} \Big[ \bar{V}^{\text{KL}}_N(\bS) \Big]$ (Eq.~\ref{eqn:svgn_avg_full}) w.r.t policy parameters $\theta$
%     \STATE Grad ascent/descent: \ $\theta \leftarrow \text{Step}_\text{adam}(\theta, \nabla_\theta \mathbb{E}_{p_\pi} \Big[ \bar{V}^{\text{KL}}_N(\bS) \Big])$; \  $\phi \leftarrow \text{Step}_\text{adam}(\phi, -\nabla_\phi \mathcal{L}^N)$
%     \ENDWHILE
%     \eindent
% \end{algorithmic} 
% \end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{enumerate}
%    \item We begin an imagined rollout from the latent state $\bS^H$ after a history of $H$ observations. We sample an action from the policy $\tilde{\bA}^H \sim \pi(.|\bS^H; \theta_{\pi})$, run this through our model to get the next prediction $\tilde{\bS}^{H+1}$, from where we sample an imagined action and so on. This gives us our imagined rollout: $\{ \bS^H, \tilde{\bA}^H, \tilde{\bS}^{H+1}, \tilde{\bA}^{H+1}, ..., \tilde{\bS}^N \}$.
%    \item We compute the reward predictions at the imagined states: $\tilde{r}^{H:N}$ and run a value backup \textbf{in the forward direction} to estimate the value for all k-step rollouts beginning from the initial state $\bS^H$: ${\tilde{V}_k = (\Sigma_{t=0}^{k-1} \lambda^k \tilde{r}^{H+t}) + V^{H+k}; k = 0:N-H}$. $\tilde{V}_k$ is the discounted sum of rewards of all intermediate states till length $k$ from the start plus the bootstrap value at the final state. \akb{If I remember correctly we used the values estimated from the true observed states (could be transition model states) so that we are not bootstrapping off of imagined values. Is this right?}
%    \item Finally, we improve the policy by maximizing the sum of these k-step value backups, $\theta_{\pi}$ is updated in the direction that maximizes $\Sigma_{k=0}^{N-H} \tilde{V}_k$. This averaging over multiple horizons is similar to SVG(0) + SVG(1) + ... SVG(N-H). Also, we additionally add a KL term (usually against a fixed prior) to the policy training objective to regularize the policy learning and prevent it from collapsing too quickly.
%\end{enumerate}


%SVG uses the value from parametric model and optimizes params to improve that value. Instead we use imagination \& bootstrap using the values from the observed encoding of the true as we don't want to bootstrap from imagined states. We use these gradients to train only the policy parameters. 

%Uses imagined observations, ILSVG, draw a schematic of the rollout with the model \& policy in latent space, how we do the horizon averaging, how that translates to a weighting of earlier states as opposed to discounted weighting which might not decay quickly enough and so on.

%write out a full algorithm that shows how the whole system works, refer to earlier equations.

%say that learning from pixels is hard, prior work has looked at doing this with latent spaces, but doing this separately is like a chicken and egg problem -- so for tasks where random exploration works this is ok but otherwise it is tricky and if you exploit too quickly it can fail too. So instead of getting data \& then latent \& then policy or random/fancy exploration policies we do interleaving all these together. In what follows we look at 3 parts of the training - model and training (mention model structure is in supplementary), value function/reward function training (structure in supplementary), policy improvement, model -> observations to latent, then intro MDP in value/reward function part in latent space, then discuss svgn + retrace, how model is used, using real rollouts. next do policy improvement, svg with imagined rollouts, n-step averaging, draw schematics maybe by hand first and put them there. Then put everything together in an algorithm, maybe mention target networks, discuss hyper params? Discuss SAC style multi-task stuff too (arch in supplementary).
%\subsection{Model Architecture and Learning:} \label{sec:model}
%\subsection{Value function and Reward Learning:} \label{sec:valuereward}
%\subsection{Policy Improvement:} \label{sec:policylearn}
%\subsection{Overall:} \label{sec:overall}



\begin{figure}
\centering
  \includegraphics[width=.9\linewidth]{figures/task/taskframes_baseandwithdist.pdf}
    \caption{\textit{Left}: \textbf{Lift-R} task - robot lifts the red block. \textit{Center-Left}: Example scene from the \textbf{Stack-B} task. \textit{Center-Right} and \textit{Right}: Tasks with unseen \textbf{distractors}. %(yellow sphere and yellow cube) added to the scene for the Lift-R and Stack-R tasks.
    }
    \label{fig:task_setup}
    \vspace{-2mm}
\end{figure}


==> Model Based RL SVGN for Robot Control/discussion.tex <==


%===============================================================================
\vspace{-.2cm}
\section{Conclusions}
\vspace{-.2cm}
We presented an approach for model-based RL where an action-conditional latent space model is trained jointly with policy, value and reward functions that operate on the learned latent space. To achieve efficient policy optimization we introduced Imagined Value Gradients (IVG), an extension of SVG (using imagined rollouts and N-step horizon averaging). We demonstrated that IVG can learn complex, long-horizon manipulation tasks like lifting and stacking. We further demonstrated in several transfer experiments on related tasks that transferring a model learned via IVG can significantly improve data efficiency compared to off-policy baselines. Crucially, transferring with models trained on multiple tasks further accelerates learning, even succeeding on tasks where single-task transfer fails.
We feel that our approach is a promising first step towards designing RL methods that combine learning of closed loop policies with the generalization capabilities that learned approximate models can provide -- although extensions (such as handling egocentric cameras, increasing sample efficiency) are needed to make our approach a fully general purpose solution for real-world robotics tasks.

%We also presented ablations and ways to accelerate performance when demonstrations from the target task are given. 
%\akb{needs a rewrite}
%We feel that our approach is a promising direction towards more general approaches and can significantly speed up learning by bootstrapping prior learned models. There is much work to be done to making our approach more data efficient for real-world tasks. There is significant work on video prediction models \cite{visual-foresight} and structured models that learn good latent representations \cite{watter2015embed, byravan2017se3}. These can be incorporated into our approach to improve sample complexity and generalization. In addition to using the learned representations models can be used as simulators, collecting experience in addition to real-world data \cite{mbrl-atari}; this significantly reduces sample complexity when an accurate model can be learned. By integrating a planner or search algorithm with a learned model we can collect targeted sequences of data that exploit the model to reach high reward states \cite{mbrl-atari, planet-dm}. Combining these trajectories with standard actor based data can lead to faster learning. Finally, exploration is a key area of research in RL; models can be used to generate useful heuristics for generating exploration data \cite{pathak2017curiosity, silver2018general}.

==> Model Based RL SVGN for Robot Control/evaluation.tex <==
\vspace{-0.2cm}
\section{Experiments} \label{sec:results}
\vspace{-0.2cm}
We evaluate our approach on several challenging long-horizon manipulation tasks in simulation (see sections D \& F of the supplementary for details). %in the Mujoco simulator \cite{todorov2012mujoco}. 
Tasks involve the agent controlling a Sawyer manipulator equipped with a Robotiq gripper with a 5-dim.\ control ($N_A $= 5) to interact with a red and blue block on a tabletop. Observations are 64x64px RGB images from two cameras located on either side of the table, looking at the robot,
and proprioceptive features.
The latent representation is 128-dimensional ($N_H$=128) and unless otherwise noted we use a history of $H=3$ observations and a rollout horizon of $N=5$.

\textbf{Task Setup: } \figref{fig:task_setup} presents visualizations of a subset of tasks from our experiments. We consider three main tasks: 1) the \textbf{Lift} task requires the robot to lift an object above a certain threshold; \textit{Lift-R} refers to lifting the red block and analagously for \textit{Lift-B}. 2) the \textbf{Stack} task requires the robot to stack one object on top of the other; \textit{Stack-R} refers to stacking the red block on top of the blue block and vice-versa for \textit{Stack-B}. 3) Lastly, the \textbf{Match Positions} task involves moving both objects to a fixed target position. We also consider variants of these tasks with the addition of \textbf{visual distractors} and \textbf{stochasticity}. It is worth noting that all our tasks involve long-term dependencies and complicated contact dynamics making them particularly challenging for model-based approaches. We use shaped rewards for all tasks except the \textit{Match Positions} task which has a mixed dense-sparse reward.

\textbf{Baselines: } We consider the following pixel-based baselines for our experiments: 1) \textbf{SVG(0)}: the model-free version of SVG. As our approach (termed Imagined Value Gradients -- \textbf{IVG} from here on out) builds on SVG we expect to improve on SVG(0). 2) \textbf{MPO}: Maximum a Posteriori Policy Optimisation \cite{abdolmaleki2018maximum}, a state-of-the-art model-free approach. To obtain an upper bound on performance we also include a version of MPO with access to the full system state (incl.\ objects). For the transfer experiments we also experiment with variants where we replace the value gradient based optimization. In particular we use \textbf{CEM}: the cross-entropy method \citep{Rubinstein:2004:CEM:1014902} using the same model as IVG for transfer (latent rollouts). \textbf{PG}: replacing the value gradients with a likelihood ratio estimator (using 100 imagined rollouts), again using the same model as used for the \emph{IVG} transfer. Additional details on the baselines are given in the appendix.

\vspace{-0.2cm}
\subsection{Learning from scratch}
We first compare IVG and the baselines when learning the Lift-R and Stack-R manipulation tasks \textit{from scratch}:
Model-based IVG(5) learns the simpler \emph{lift} task stably and performs on par with the baselines (\figref{fig:scratch_results}, left). 
On the harder stack task (\figref{fig:scratch_results}, right), IVG(5) learns significantly (about 2x) faster than both MPO and SVG(0), and also outperforms SVG(0) in terms of final performance.
Compared to the informed MPO (State) baseline, IVG learns more slowly, but this difference is significantly reduced for stacking. Even when learning from pixels, the structure inherent in IVG via the latent space rollouts allows it to learn complex tasks faster than strong model-free baselines. 

We also tested the ability  of IVG to handle slightly more stochastic and partially observed environments.
\figref{fig:scratch_results} (right) presents results on learning the Stack-R task in environments with: 1) delayed proprioception (2 timestep lag) and 2) noisy observations where one of the blocks switches colors randomly every 3 frames. IVG(5) successfully learns in both cases (albeit more slowly). MPO also solved these tasks but required approximately $2x$ more episodes than IVG (color switch not shown).


\begin{figure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/lift_ivgn.pdf}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/stack_ivgn.pdf}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/noisy_observation_stack.pdf}
\end{subfigure}
\caption{\textit{Left}: IVG(5), with $N=5$, performs similarly to the model-free baselines MPO and SVG(0) on the \textbf{lift} task. Black dotted line represents MPO (state) scoring higher than a reward threshold indicating success (300 for Lift, 140 Stack) for 50 episodes. \textit{Center}: IVG(5) learns significantly faster than SVG(0) and MPO on the \textbf{stack} task. \textit{Right}: IVG(5) learns well even in environments with noisy observations.}
\label{fig:scratch_results}
\vspace{-0.5cm}
\end{figure}


%and the Stack-R task on two additional stochastic environments (right) with delayed proprioception (2 step lag) and switching of colors. 

%We first evaluate the performance of our proposed RL algorithm (termed Imagined Value Gradients -- IVG from here on out) on two tasks: the \textbf{Lift-R} task has a red and blue block on the table, the task is to always lift the red block above a certain height; the \textbf{Stack-R} task involves stacking the red block on top of the blue one.\footnote{The Lift-B task is to lift the blue block and similarly for stacking.} We used a shaped reward for both tasks. We train IVG from scratch on both these tasks with a rollout length of $N=5$ and a history of $H=3$ observations, labeled IVG(5). We compare against the following baselines: 1) SVG(0), the model-free off-policy version of SVG; 2) Maximum a Posteriori Policy Optimisation (MPO) \cite{abdolmaleki2018maximum}, a state-of-the-art model-free baseline trained on image observations and proprioception (MPO); and 3) MPO using the true state of the system, mainly to get an idea of the difficulty of the learning problem. 

%\figref{fig:results_base} shows the results on these two tasks, demonstrating that IVG is capable of learning stably on complex manipulation tasks. On the lift task (\figref{fig:results_base}, left) all image-based methods perform similarly; IVG(5) can match the performance of the baselines while also learning a model and performing imagined rollouts through the learned model. The difference is more stark on the stack task (~\figref{fig:results_base}m right), IVG(5) learns faster than both MPO and SVG(0) showing that the model does help improve performance on a complicated manipulation task.% which requires significantly more exploration. 

%\subsection{Multi-task learning}
%\akb{Maybe a paragraph instead of a sub-section?}
%\textbf{Multi-task learning:} A model trained on multiple tasks should transfer better than one from a single task due to the diversity in transitions observed. To test this hypothesis, we trained a multi-task variant of IVG using the SAC framework\cite{riedmiller2018learning} on the Stack-R task. The intrinsic rewards (or sub-tasks) included tasks such as Reach-R, Lift-R, Move-R etc. We additionally added a Reach-B sub-task to allow the model some experience with the blue block. \figref{fig:transfer_results} (center) shows the results when this learned model is used for transfer learning on the Stack-B task. The multi-task version of IVG significantly outperforms all other methods including IVG trained on Stack-R. This demonstrates the capability of the model to distill information from multiple tasks and the potential of multi-task learning to transfer quickly on new related tasks. We present additional results on multi-task learning in the supplementary.

\vspace{-0.2cm}
\subsection{Transferring learned models to related tasks}
IVG learns a model of the environment which we may be able to transfer, and thus accelerate learning of related tasks. In the following, we evaluate this possibility.
First, we train IVG from scratch on one or multiple source task(s). 
Second, we copy the weights of the trained model (\textbf{encoder} $f_\text{enc}$, \textbf{transition} model $f_\text{trans}$ and \textbf{decoder} $f_\text{dec}$). The policy, value and reward models are not transferred and are learned from scratch.
%We then use the previously copied weights to initialize the model parameters when training on the target task, whose performance is reported in the experiments. 
As a model-free baseline we include MPO where we initialize all weights of the policy \& value function except the last layer from an agent trained on a source task.
%A major advantage of IVG, in comparison to model-free methods, is that we learn a model of the environment; this model can be used to accelerate learning on related tasks. In the following, we evaluate the transfer capability of models learned using IVG. Briefly, transfer happens in three steps: 1) First, we train IVG from scratch on a source task (or multiple source tasks). 2) Second, we copy the weights of the trained model, specifically of the \textbf{encoder} $f_\text{enc}$, \textbf{transition} model $f_\text{trans}$ and \textbf{decoder} $f_\text{dec}$. The policy, value and reward models are not transferred and are learned from scratch. 3) We use the previously copied weights to initialize the model parameters when training on the target task, whose performance is reported in the experiments. As an additional baseline, we train a version of MPO where we initialize all weights of the policy \& value function (except the last layer) from an agent trained on a prior source task.

\textbf{Multiple source tasks: } A model trained on multiple tasks should transfer better due to the diversity in transitions observed. To test this hypothesis, we propose a version of IVG that is trained on multiple source tasks -- learning a task agnostic model. We use the following source tasks: Reach-B, Move-B, Lift-B, Stack-B and Reach-R (most tasks involve the blue object but Reach-R gives  the
model some experience with the red block). Details on this setup are provided in the supplementary.

\textbf{Transfer results: } We present results on transferring IVG models to the following target tasks: 

%1) \textbf{Lift-R: } \figref{fig:transfer_results} (left) shows the transfer performance of IVG(5) on the Lift-R task. When transferring from the source task \textit{Stack-B}, IVG(5) learns $\sim$2x faster compared to learning from scratch and $\sim$4x faster than MPO (irrespective of whether it is pre-trained or not). Furthermore, transferring IVG(5) from the source task \textit{Stack-R} accelerates learning further as the model has already observed many relevant transitions, achieving speed comparable to the state-based version of MPO. Both these results highlight the significant benefits of a model when transferring to related tasks, even in cases where the model has only observed a subset of relevant transitions. 
1) \textbf{Lift-R: } \figref{fig:transfer_results} (left) shows the transfer performance of IVG(5) on the Lift-R task. With a model pre-learned on \textit{Stack-B}, IVG(5) learns $\sim$2x faster than from scratch and $\sim$4x faster than MPO (irrespective of MPO's initialization). A model pre-trained on \textit{Stack-R} accelerates IVG(5) further since the model has already observed many relevant transitions, achieving speed comparable to \emph{MPO (state)}. Replacing the learned policy with direct optimization (\emph{CEM}) or using a policy gradient yields sub-optimal behavior. These results highlight the benefits of a model when transferring to related tasks, even in cases where the model has only observed a subset of relevant transitions. 


%2) \textbf{Stack-R: } Similar to the results on the Lift-R task, IVG with transferred models learns much faster on the Stack-R task (\figref{fig:transfer_results}, center). In addition to transfer from \textit{Stack-B}, we also compared the performance when transferring from a model trained on multiple source tasks (\textit{Multitask}). Crucially, this multi-task variant significantly accelerates learning speed; it is $\sim$1.5x faster than transferring from a single-task and about $\sim3x$ faster than learning from scratch. As we will see from subsequent results, models trained on multiple tasks greatly accelerate transfer.
2) \textbf{Stack-R: } Results with transferred models for Stack-R are similar to those for Lift-R (\figref{fig:transfer_results}, center). But here, \emph{CEM} fails to perform the stack (possibly caused by overly exploiting the model due to missing policy regularization), and using \emph{PG} instead of a value gradient takes significantly longer to converge (15k trajectories) and performs worse, likely due to the noise in the likelihood ratio calculation -- even though we already used 100 forward rollouts for the likelihood ratio calculation (1 for IVG), a $25$ fold increase in computation. In addition, we also compared the performance when transferring a model trained on multiple source tasks (\textit{Multitask}). This multi-task variant significantly accelerates learning speed; it is $\sim$1.5x faster than transferring from a single-task and about $\sim3x$ faster than learning from scratch. As we will see from subsequent results, models trained on multiple tasks greatly accelerate transfer.


3) \textbf{Match Positions: } We tested model generalization on the \emph{match positions} task, which differs significantly from the source tasks (\figref{fig:transfer_results}, right). All agents except  multi-task IVG fail on this task; this includes transferring IVG from a single task (Stack-B) and the pixel-based MPO. This is likely due to the sparse structure of the reward (see supplementary). This shows how multi-task training enables the formation of robust and expressive latent spaces that transfers well to new tasks.


%3) \textbf{Match Positions: } We tested the generalization of our learned models on the match positions task, a task with different reward structure than all prior tested tasks (\figref{fig:transfer_results}, right). All agents except the one transferring from multi-task IVG fail on this task; this includes transferring IVG from a single task (Stack-B) and the pixel-based MPO. We believe this is due to the sparseness of the reward; significant exploration is needed to figure out the reward substructure.  This further demonstrates the benefits of multi-task learning; representations learned on multiple tasks need to be predictive of diverse rewards and values, this enables robust and expressive latent space learning.

%\textbf{Visual distractors: } Lastly, we analyzed the generalization of IVG in the presence of visual distractors; \figref{fig:distractor_ablation}, (left \& center) presents results when a yellow cube or ball are added to the scene. IVG, when transferring from single or multiple source tasks is still able to learn stably on these tasks (as does IVG from scratch). The multi-task transfer version of IVG significantly outperforms all other methods, learning $\sim$3x faster than from scratch and $\sim$4x faster than MPO. This is a surprising result as CNNs are known to be sensitive to changes in visual inputs; jointly training a model with the policy allows it to optimize for task performance in addition to prediction and reconstruction, leading to more robust representations that can transfer quickly. 

4) \textbf{Visual distractors: } Lastly, we analyzed the generalization of IVG when visual distractors in the form of a yellow cube or ball are added to the scene (\figref{fig:distractor_ablation}, (left \& center)). Transfer from one or multiple source tasks remains effective. Transferring a multi-task model significantly outperforms all other methods, learning $\sim$3x faster than from scratch and $\sim$4x faster than MPO. Thus, even though CNNs are known to be sensitive to changes in visual inputs, jointly training a predictive model with the policy  can still lead to robust representations that transfer quickly. 



%Finally, we test the transfer performance of IVG when a third object of unseen color (and shape) is introduced into the scene. \figref{fig:distractor_ablation}, left \& center plots present results when a yellow cube or sphere is added to the scene respectively. Even in the presence of these visual distractors, IVG when transferring outperforms the baselines. \akb{Write this better?} %This is a surprising result as convolutional neural networks are known to be sensitive to changes to visual inputs, even with addition of noise \cite{nguyen2015deep}. We plan to further explore this in future work.

%We further explored the transfer capabilities of IVG by transferring models learned on stacking the blue block (Stack-B) to the Stack-R task (\figref{fig:transfer_results}, center); this once again leads to significant boost in performance

%IVG(5) when transferring from a source task is significantly faster than training from scratch and the transfer version of MPO. While the performance improvements are not as drastic as the lift setting since there is a larger mismatch between the model's experience and the target task, there is a consistent increase in learning speed when we transfer learned models.
%This boost in learning speed is further exacerbated in a \textit{re-learning} setting, as evidenced when transferring from the source task \textit{Stack-R}; as the model has already observed many relevant transitions we see an additional $\sim$2x improvement compared to the Stack-B transfer setting. This speed is comparable to training MPO from state (using true block positions instead of images); further demonstrating the strength of the learned model.


%This highlights the significant benefits of a model when transferring to related tasks, even in cases where the model has only observed a subset of relevant transitions.

%Furthermore, transferring IVG(5) from the source task \textit{Stack-R} accelerates learning further, achieving comparable speed to the state-based version of MPO; it is worth noting that this is 

%\textbf{Lift-R:} \figref{fig:transfer_results} (left) shows the transfer performance of IVG(5) on the Lift-R task. When transferring with a model trained on the Stack-B task, IVG(5) experiences significant speed-ups compared to the baselines. It is $\sim$2x faster compared to training from scratch and $\sim$4x faster than MPO . This highlights the significant benefits of a model when transferring to related tasks, even in cases where the model has only observed a subset of relevant transitions. This boost in learning speed is further exacerbated in a \textit{re-learning} setting as can be seen in the learning curve when we transferred a model trained on Stack-R to Lift-R; as the model has already observed many relevant transitions we see a $\sim$2x improvement in learning speed compared to the Stack-B transfer setting. This speed is comparable to training MPO from state (using true block positions instead of images); further demonstrating the strength of the learned model.

%This does provide the multi-task learner an advantage, but also showcases the strengths of learning on multiple tasks.

%A major advantage of IVG, in comparison to model-free approaches, is that we learn a model of the environment; this model can be used to transfer to related tasks. 

%Next, we present results where we transfer learned IVG models (on source tasks) to a related target task. For these experiments, we initialize the weights of the encoder, decoder and transition networks for the target transfer task from the models learned on the source task; the policy, value and reward models are all trained from scratch. In addition to the baselines from above, we also train a version of MPO where we initialize the weights of the policy (except the last layer) from an agent trained on a prior source task. \\

\begin{figure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/transfer_lift.pdf}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/transfer_multitask_stack.pdf}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/transfer_match_positions.pdf}
\end{subfigure}
\caption{Transfer performance of IVG(5) on various target tasks. Task names inside square brackets indicate the source task. \textit{Left}: Transfer results on Lift-R. Transferring from Stack-B leads to large improvements compared to baselines. \textit{Center}: Transfer from multi-task IVG outperforms all baselines and single-task IVG. \textit{Right}: Multi-task IVG successfully transfers on the Match Positions task while single-task IVG and other baselines fail.}
\label{fig:transfer_results}
\vspace{-2mm}
\end{figure}


\begin{figure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/transfer_lift_distractor.pdf}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/transfer_stack_distractor.pdf}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/results/comparison_n_stack.pdf}
\end{subfigure}
\caption{\textit{Left \& Center}: Transfer performance on the visual distractor task where a yellow block or ball are added to the Lift-R and Stack-R task respectively. 
transfer from multi-task IVG leads to a $\sim$3-4x speedup \textit{Right}: Ablation tests with IVG, using horizon lengths of $N=0,1,5,20$ \& using a single N-step horizon for computing the policy gradient (Eq.~\eqref{eqn:svgn_theta} instead of Eq.~\eqref{eqn:svgn_avg_full}). 
IVG(0) uses the model loss (with horizon 5) only as an auxiliary signal (and otherwise corresponds to SVG(0)). 
}
\label{fig:distractor_ablation}
\vspace{-2mm}
\end{figure}

%\textbf{Lift-R:} \figref{fig:transfer_results} (left) shows the transfer performance of IVG(5) on the Lift-R task. When transferring with a model trained on the Stack-B task, IVG(5) experiences significant speed-ups compared to the baselines. It is $\sim$2x faster compared to training from scratch and $\sim$4x faster than MPO (irrespective of whether it is pre-trained or not). This highlights the significant benefits of a model when transferring to related tasks, even in cases where the model has only observed a subset of relevant transitions. This boost in learning speed is further exacerbated in a \textit{re-learning} setting as can be seen in the learning curve when we transferred a model trained on Stack-R to Lift-R; as the model has already observed many relevant transitions we see a $\sim$2x improvement in learning speed compared to the Stack-B transfer setting. This speed is comparable to training MPO from state (using true block positions instead of images); further demonstrating the strength of the learned model.

%\textbf{Stack-R:} We further explored the transfer capabilities of IVG by transferring models learned on the Lift-R and Stack-R task to the Stack-B task (\figref{fig:transfer_results}, center). Even in this setting, the learned model provides a boost to learning; IVG(5) when transferring from a source task is significantly faster than training from scratch and the transfer version of MPO. While the performance improvements are not as drastic as the lift setting since there is a larger mismatch between the model's experience and the target task, there is a consistent increase in learning speed when we transfer learned models.

%\textbf{Match positions:} We designed a task with significantly different reward structure to test the generalization capabilities of our learned models. The \textbf{push} task requires the agent to push both blocks to a fixed target position, with a reward measuring based on the distance to the target position. Unlike prior tasks, this task has a mixed sparse-dense reward where the reward remains constant until the blocks are moved. \figref{fig:transfer_results} (right) shows the performance of various algorithms on this task. All agents except the multi-task IVG fail to solve the task due to the sparseness of the initial reward; significant exploration is needed to figure out the reward substructure.  This further demonstrates the benefits of multi-task learning; the learned representations need to capture the reward and value structure of multiple related tasks, potentially leading to better shaped latent spaces.

%\textbf{Visual distractors:} Finally, we test the transfer performance of IVG when a third object of unseen color (and shape) is introduced into the scene. \figref{fig:distractor_ablation}, left \& center plots present results when a yellow cube or sphere is added to the scene respectively. Even in the presence of these visual distractors, IVG when transferring outperforms the baselines. \akb{Write this better?} %This is a surprising result as convolutional neural networks are known to be sensitive to changes to visual inputs, even with addition of noise \cite{nguyen2015deep}. We plan to further explore this in future work.
\vspace{-0.2cm}
\subsection{Ablation experiments}
\label{sec:ablation}
%\akb{Note: corresponding plots still missing}
% We further analyzed the performance of IVG with two ablations, evaluating our design choices:

% \textbf{Rollout horizon: } To evaluate the effect of the rollout horizon $N$, we tested IVG across multiple settings of $N$=0,1,5,20. \figref{fig:distractor_ablation} (right) presents these results, evaluated on learning the Stack-R task from scratch; in general IVG is robust to the choice of the rollout horizon, i.e. IVG learns stably for all settings of $N$ we tried. Interestingly, the choice of $N$ has a marked effect on the speed of learning, smaller values $N$=0,1 tend to learn slowly; increasing $N$ speeds up learning dramatically (see $N$=5) upto a point after which there is a potential slowdown. 

% \textbf{Averaging value gradients: } To quantify the effect of averaging value gradients across multiple rollout horizons \eqref{eqn:svgn_avg_full}, we ran experiments using a single imagined rollout of length $N$. \figref{fig:distractor_ablation} (right) presents these results; for short horizons e.g. $N$=5, using a single rollout horizon leads to lower learning. On the other hand, learning completely fails for longer horizons $N$=20 (unlike with averaging) potentially due to cascading model errors on imagined rollouts, validating our approach.

To validate our algorithm and model design choices we performed two sets of ablations.\\
\textbf{Rollout horizon: } To evaluate the effect of the rollout horizon $N$ on the policy gradient (eq.~ \eqref{eqn:svgn_theta}) we tested IVG across multiple settings of $N$=0,1,5,20 for learning \emph{Stack-R} from scratch ( \figref{fig:distractor_ablation} (right)). IVG is robust to the choice of the rollout horizon and learns stably for all settings of $N$. However, the choice of $N$ has a marked effect on the speed of learning. Increasing $N$ speeds up learning up to a point after which no additional speedup is obtained (compare $N=0,1,5$). Importantly, these results suggest that the benefit of the model in IVG is not just one of representation learning in partially observed domains but that using the model for policy optimziation is beneficial.\\
\textbf{Averaging value gradients: } To quantify the effect of averaging value gradients across multiple rollout horizons (c.f. Eq \eqref{eqn:svgn_avg_full}), we ran experiments using a single imagined rollout of length $N$ ( \figref{fig:distractor_ablation}, right). For short horizons e.g. $N$=5, using a single rollout horizon leads to lower learning speed. On the other hand, learning completely fails for longer horizons $N$=20 (unlike with averaging) potentially due to cascading model errors on imagined rollouts, validating our averaging approach.


% Note that IVG(0) uses the model loss (rollout length of 5), only as an auxiliary signal -- and learns a Q-function for policy optimization akin to SVG(0).

%namely, the choice of the rollout horizon $N=5$ and the effect of averaging value gradients across multiple horizons \eqref{eqn:svgn_avg_full}: 

%: 1) To quantify the effect of the proposed N-step horizon averaging we performed an ablation where we used a single horizon of length $N$. \figref{fig:distractor_ablation} (right) shows the results; in practice horizon averaging works significantly better and is more stable compared to using a single horizon which can occasionally fail to learn due to compounding model errors.
%2) We looked at varying the rollout horizon of IVG ($N$), while keeping the history ($H$) fixed. We tried $N = 2, 5, 10, 20$ and found that a length of $N=5$ gave the best results. (see ~\figref{fig:distractor_ablation} (right)) Shorter horizons were significantly slower during learning while using longer horizons didn't significantly impact performance (validating our N-step horizon averaging) except for a significant slowdown on the learner due to the length of the rollouts.



%\item We also analyzed the effect of the gradient from the value and reward losses on the model learning by performing an ablation where we stopped the gradient flow from these losses back to the model. \figref{fig:ablationstodo} (right) shows the performance of this model on the source tasks. In practice this does not perform as well compared to the alternative; training the latent state to be predictive of value and reward adds better shaping during the learning process leading to better final representations.

%\subsection{IVG + Expert demonstrations}
%\akb{Note: Experiment needs to be run \& corresponding plots  missing}
%Lastly, we explored the role of exploration in fast learning and transfer by training an IVG agent that has access to a few expert demonstrations on the target task. \figref{fig:explorationtodo} presents the results when we added 10, 100 and 1000 expert demonstrations to the replay buffer. With access to the demonstrations IVG and baselines are able to discover the underlying reward structure much faster leading to a significant speed up in learning. Even in the transfer setting where there is a pre-trained model exploration can drastically accelerate learning; one of the major bottlenecks in transfer is the discovery of the reward structure on the new task, with this knowledge the policy can be learned very quickly. Exploration is still one of the major challenges for data-efficient RL, much work is needed in this area.

==> Model Based RL SVGN for Robot Control/introduction.tex <==
%===============================================================================
\section{Introduction}
\vspace{-0.2cm}
The last decade has seen significant progress in reinforcement learning. The field has matured to a state where RL can solve challenging simulated motor control problems \cite{heess2017emergence, openai2018} or games  \cite{silver2018general,alphastarblog} even from high-dimensional observations such as images \cite{mnih2015human, mbrl-atari,espeholt2018impala}. 
Off-policy model-free algorithms have become workable for high-dimensional continuous action spaces %and motor control tasks
\cite{lillicrap2015continuous,heess2015learning,abdolmaleki2018maximum}, and have improved in robustness and data-efficiency allowing experiments directly on robotics hardware
\cite{abdolmaleki2018relative,haarnoja2018soft,zhu2018, kalashnikov2018qt}.

Model-free techniques directly learn a policy (and value function) from environment interactions. Their simplicity, generality and versatility has been a major factor behind their recent successes. 
%\akb{Does not flow well (in the rest of the para) from here on}
Yet, these techniques do not entirely satisfy the intuition that a learning agent should be able to acquire approximate knowledge of the dynamics of its environment in a manner that is independent of any particular task and such that it is easily applicable to new tasks, more easily than task-specific objects such as policies. It is this intuition and as well as the desire to further improve the sample-efficiency and transferability of solutions that has driven much of the recent research in model-based RL.
% %, and be able to leverage this knowledge to improve its behavior. 
% Such knowledge would then be transferable to new tasks in the same domain more effectively than task-specific objects such as policies. It is this intuition and, more practically speaking, the desire to further improve on the sample-efficiency and transferability of model-free solutions that has driven much of the recent research in model-based RL.

A growing body of literature is concerned with learning dynamics models for physical control problems \cite{deisenroth2011pilco,visual-foresight}, including approaches that learn latent models from images \cite{watter2015embed,planet-dm,solar-icml19}. Although some approaches excel in data efficiency  \cite{deisenroth2011pilco,levine2016end}, in general, model-based methods have not yet achieved the robustness of model-free techniques; and they still struggle with model inaccuracies and long planning horizons. When learned dynamic models are combined with policy learning \cite{sutton1990integrated,gu-modelbasedacc,imagination-dm,mve-feinberg,wayne2018unsupervised} the advantages over purely model-free techniques can be less clear. 


%In some cases it has been possible to achieve very data efficient control with such approaches \cite{XYZ,ABCTODO}. 
%In general, such model-based approaches have, however, not yet been able to achieve the same robustness and versatility as model-free techniques due to problems in the presence of model inaccuracies. 

%\tobi{removed the paragraph on lots of related work here as I think we have this down in the related work already it is only commented out though}
%There has been a number of works exploring learned dynamics models for physical control problems \cite{XXX} including approaches that employ latent dynamic models and are hence capable to operate in domains when the system is observed e.g. through images \cite{XYZ}. Although in some cases it has been possible to achieve very data efficient control \cite{XYZ}, these approaches often dispense of a policy and rely on model predictive control (i.e.~rely on planning through the model) at test time. This can, however, lead to problems in the presence of model inaccuracies, or when a task is defined by sparse rewards or requires a long planning horizon. More generally, such model-based approaches have not yet been able to achieve the same robustness and versatility as model-free techniques. 
% planning horizon, model quality
%\akb{This is isolated, maybe start with saying there has been work in the intersection but advantages are not clear?}
%There has also been work combining learned dynamic models with policy learning \cite{xxx}, however, in such cases the advantages over purely model-free techniques are often less clear. 

In this work we develop an approach that uses model-based RL to learn a stochastic parametric policy in domains with high-dimensional observation spaces such as images. We build on Stochastic Value Gradients (SVG) \cite{heess2015learning} which allow us to compute low-variance policy gradients by directly differentiating a model-based value function.
We extend this work in two ways: Firstly, we develop a latent state space model that allows us to predict expected future reward and value as a function of the current policy even when the true low-dimensional system state is not directly observed. Secondly, rather than using the model only for credit assignment along observed trajectories we use it directly to produce ``imagined'' rollouts and show that stable policy learning can still be achieved.

We apply our algorithm to several challenging long-horizon vision-based manipulation tasks (e.g.~lifting and stacking) in simulation and demonstrate the following:
Our model-based approach (a) is as robust and achieves the same asymptotic performance as competitive model-free baselines, and (b) in several cases it significantly improves data-efficiency. (c) It can effectively transfer the learned model to novel tasks with different reward distributions or visual distractors, leading to a dramatic gain in data-efficiency in such settings. (d) It is particularly effective in a multi-task setup where the models learned on multiple tasks learn faster and generalize better to new tasks, successfully solving problems that cannot be learned in isolation.




% Reinforcement Learning (RL) has recently seen tremendous success on many challenging control problems \cite{deisenroth2013survey, kober2013reinforcement}, even when learning directly from images \cite{mnih2015human, lillicrap2015continuous, mbrl-atari}. In particular, model-free RL methods for robotics (where one learns a policy directly mapping states to actions) have significantly matured and are now capable of generating state of the art results on complex, long-horizon manipulation tasks in contact-rich environments \cite{lillicrap2015continuous, schulman2017proximal, riedmiller2018learning}. In spite of these advancements, several key challenges exist that limit their applicability. Firstly, the poor sample complexity of model-free RL means it requires large amounts of real-world interaction. More importantly, model-free methods transfer poorly; the learned policies are task-specific and hard to transfer even on related tasks.

% %requires large amounts of data to learn, leading to poor data efficiency. Second, model-free methods transfer poorly; the learned policies, value and reward functions are task-specific and cannot be used to quickly transfer across tasks. 

% In contrast to model-free RL, model-based approaches estimate the (expected) dynamics of observations and in some cases, rewards and values. This can lead to improved data efficiency \cite{deisenroth2011pilco, levine2016end} and crucially, fast adaptation when transferring to related domains \cite{sutton1990integrated}. Traditionally these methods were limited to state-space tasks, but with the advent of deep learning there has been significant progress on learning image-based predictive models \cite{xue2016visual, byravan2017se3, ebert2018visual} and (structured) low-dimensional latent representations \cite{watter2015embed, planet-dm}, leading to model-based RL being applied to continuous visual control tasks \cite{watter2015embed, wahlstrom2015pixels, planet-dm, solar-icml19, ke2018modeling, cobra-dm}, Atari games \cite{mbrl-atari} and tabletop manipulation \cite{ebert2018visual}. One drawback of many of these approaches is their reliance on planning through the learned model for generating actions at execution time, which can both be difficult in the presence of model errors (e.g. on long-horizon tasks and sparse reward tasks), and expensive in terms of computation.

% In this paper, we explore a way to combine the strengths of a model-based approach with stable learning of parametric policies via RL that \emph{is particularly suited for fast transfer to related domains}. To this end, we estimate an action-conditional expectation model of the observations -- and the reward -- in tandem with a low-variance gradient based policy optimization approach derived from the perspective of Stochastic Value Gradients (SVG) \citep{heess2015learning}. We extend SVG to use imagined rollouts and use averaging of returns over multiple rollout horizons to reduce model approximation errors. Our model learns a deterministic mapping of observations to abstract, latent states, evolving the transition dynamics in this low-dimensional representation and reconstructing observations, (expected) rewards and %(expected) 
% values from this latent state. We train the model jointly alongside the policy which operates on the learned latent state as opposed to raw observations. We test our approach on complex, simulated, long-horizon manipulation tasks (e.g. lifting, stacking) and show comparable performance to standard model-free benchmarks.
% %TODO: next sentence should go into related work
% %While there has been significant work at the intersection of model-free and model-based RL \cite{sutton1990integrated, gu-modelbasedacc, imagination-dm, mve-feinberg}, even involving latent representation learning \cite{gelada2019deepmdp, franccois2018combined, oh2017value}, there is very little work that explores the use of these learned models for transfer learning (with the exception of \cite{sutton1990integrated, franccois2018combined} which show transfer on toy problems). 
% We then show that our approach can leverage the learned model for fast transfer to multiple associated manipulation tasks, achieving significant speed ups on tasks with different reward distributions and visual distractors. We also evaluate a multi-task variant of our approach; models learned on multiple tasks learn faster and generalize better to new tasks, successfully solving a mixed sparse and dense reward task where single-task learning fails. 
% %Lastly, we highlight the importance of exploration by showing significant speed-ups in transfer learning when a few demonstrations of the target task are available; while an environment model can accelerate transfer, our agent still needs to explore to observe rewards during learning. 

% \akb{I think we really need to nail down on the transfer aspect and how using a model enables multi-task learning to be more powerful and vice-versa where training a model in the multi-task setting leads to much better transfer.}


% %Model-free Reinforcement learning (RL) has recently seen tremendous success on challenging problems \cite{deisenroth2013survey, kober2013reinforcement}, achieving human level performance in Atari games \cite{mnih2015human}, beating the world champion at Go \cite{silver2018general}, and generating state of the art results in non-linear control and manipulation tasks in contact-rich environments \cite{lillicrap2015continuous, schulman2017proximal, riedmiller2018learning}. With recent advances in deep learning \cite{krizhevsky2012imagenet}, these methods can now scale to high-dimensional state and observation spaces \cite{mnih2015human, riedmiller2018learning}, often representing policies, value, Q-value and reward functions as large neural networks with potentially millions of parameters. In spite of these advancements, several key challenges exist that limit their applicability to general real world robotics tasks. First, model-free RL requires large amounts of data to learn, leading to poor data efficiency. Second, model-free methods transfer poorly; the learned policies, value and reward functions are task-specific and cannot be used to quickly transfer across tasks. These issues can be mitigated to a certain extent by estimating a model of the environment \cite{sutton1990integrated}. 

% %Model-based RL approaches learn a predictive model of the future and use this model to act in the environment. Prior work on model-based RL has shown impressive data efficiency \cite{deisenroth2011pilco}, even in contact-rich manipulation settings \cite{levine2016end}. These methods have recently been extended to handle high-dimensional visual observations \cite{watter2015embed, wahlstrom2015pixels, ebert2018visual, planet-dm, solar-icml19, ke2018modeling, cobra-dm}, primarily through the use of neural networks. Furthermore, models can be used to quickly transfer across domains where the transition dynamics are similar. A major drawback of these methods is their reliance on the model to generate accurate predictions of the future; when the model approximation error is high these methods tend to perform poorly or fail completely \cite{}. Additionally, many of these methods rely on a forward planning algorithm (such as iLQR~\cite{todorov2005generalized}, CEM~\cite{rubinstein2013cross}) to generate policies; planning can be difficult for long-horizon tasks with sparse rewards.

% %\akb{Do we need this? Maybe shrink this a bit? This is pretty much the same as the abstract.}
% %Our contributions are:
% %\begin{enumerate}
% %    \item We propose a hybrid RL agent that learns a latent representation from visual observations, latent transition dynamics and policies that operate in the learned latent space (Sec.~\ref{sec:arch}). 
% %    \item We propose ILSVG (Imagined-Latent-SVG), an extension of SVG which use imagined rollouts in a learned latent space for policy optimization (Sec.~\ref{sec:policylearn}). ILSVG uses averaging over multiple rollout horizons to reduce the effect of model approximation errors.
% %    \item We empirically evaluate ILSVG on a set of simulated long-horizon manipulation tasks such as lifting and stacking. We also evaluate a multi-task variant of ILSVG that uses the Scheduled Auxiliary Control (SAC) \cite{riedmiller2018learning} framework (Sec.~\ref{sec:results}).
% %    \item Finally, we show transfer results on finetuning previously learned models on tasks with different reward structures and visual distractors; we also discuss performance improvements when a few demonstrations from the target task are available (Sec.~\ref{sec:results}).
% %\end{enumerate}

% %Talk about latent space models, how we use our model to learn latent space directly from images for control. Finally talk about transfer learning, and how there has not been much results of that. Last, mention contributions.

% %More recent work has further explored the use of imagined rollouts through learned models for improving the sample efficiency of model-free learning, using locally-linear models \cite{gu-modelbasedacc} and imagined trajectory inputs to actor-critic methods \cite{imagination-dm}. Model-based imagined rollouts have also been used to bootstrap better value estimates to speed up value function based learning \cite{mve-feinberg, steve-nips19}. In contrast to these methods, the Stochastic Value Gradients (SVG) approach \cite{heess2015learning} uses a learned model for generating rollouts of off-policy data from prior experience, accelerating learning through value gradients backpropagated via the learned model. Our approach extends 

% %Model-free RL, survey, networks, advantages, disadvantages. Major challenges. Models - issues, model based exmaples, NNs, combining the two has advantages, talk about different ways to do that in literature, what do we do?

% %Why models? How can they help? RL advantages vs Planning
% %Our contributions include:


==> Model Based RL SVGN for Robot Control/related.tex <==
%===============================================================================
\vspace{-0.2cm}
\section{Related Work}
\vspace{-0.1cm}
%\akb{Do we need this section? A lot of this is discussed above in the intro.}\\
%\akb{We can add a section on latent space models here if we decide to focus more on models + transfer. Might make more sense.}
%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Model-free RL:} Model-free RL has recently been applied to many challenging problems including robotics \cite{deisenroth2013survey}. These successes were
helped by advances in algorithms suitable for the use of powerful function approximators \cite{mnih2015human, lillicrap2015continuous, schulman2017proximal, abdolmaleki2018maximum, silver2018general, riedmiller2018learning}, also enabling the use of RL in domains with high-dimensional observation spaces \cite{mnih2015human, alphastarblog, riedmiller2018learning}.
However, model-free methods can still struggle in the low data regime and their primary objects of interest, policies and value functions are task specific and can thus be difficult to transfer.

%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Model-based RL:} On the other end of the spectrum, model-based methods learn a model of the environment and use a planner to generate actions. One of the successes in this area is work by Deisenroth et al. \cite{deisenroth2011pilco} who learn uncertainty aware policies using Gaussian-Process models and showed impressive data efficiency on multiple low-dimensional tasks. Using deep neural networks, model based RL has been extended to vision-based problems such as Atari \cite{mbrl-atari} and complex manipulation tasks \cite{levine2016end, visual-foresight}. Other work has studied learned vision-based latent representations for RL \cite{watter2015embed, wahlstrom2015pixels, solar-icml19, cobra-dm, planet-dm}: Such low-dimensional representations 
%can provide good, task-specific, 
can provide feature spaces in which learning and planning can proceed significantly faster compared to learning directly from images 
% However, problems
% %While these approaches generate impressive results, they often struggle 
% with model inaccuracies and on tasks with sparse rewards and long-horizons remain.
although model inaccuracies, sparse rewards, and long-horizons remain challenging.

%\cite{visual-foresight} learns a video prediction model based on self-supervised training data, primarily generated through random exploration followed by CEM style planning with different reward function specifications (pixel error, goal images and goal classifiers).

%\citep{planet-dm} is another model-based RL method that learns a latent state representation from pixels and uses the CEM for planning in the learned latent space. The learned model has both stochastic and deterministic components and is trained to minimize long-term prediction error. The method is tested on visual control tasks in mujoco.

%\citep{solar-icml19} is a purely model-based RL method that learns a state representation from images that can be used in conjunction with iLQR style controllers (similar to E2C). The approach is tested on real world stacking tasks where the block is already grasped \& the target position is fixed. It is also trained on a real-world pushing task.

%\citep{ke2018modeling} is also a model-based RL approach that learns a predictive model with an auxiliary loss for consistent long-term future predictions. This mode is then used in conjunction with an MPC style planner and a PPO style optimization algorithm for learning exploration policies. It is tested on mujoco tasks with visual observations.

%\citep{cobra-dm} from DeepMind learns a representation along with a 1-step transition model, exploration policy and reward predictor for simple 2D object movement tasks. Uses the MONet architecture for representation learning. \\

%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Model-free + Model-based:} Several papers have focused on combining the strengths of model-free and model-based RL. The work on Dyna \cite{sutton1990integrated} was among the first. It integrates an action model and model-based imagined rollouts with policy learning, interleaving planning, learning and execution in a tight loop. Recent work has further explored the use of imagined rollouts generated with learned models for accelerating learning of model-free policies \cite{gu-modelbasedacc, imagination-dm} -- or indirectly speeding up learning via model-based value estimates \cite{mve-feinberg, steve-nips19}. These approaches propose different means to handle model approximation errors, such as using short rollouts to avoid cascading model errors \cite{mve-feinberg}, uncertainty estimation through model ensembles \cite{steve-nips19} and using the rollouts as policy conditioning variables only \cite{imagination-dm}. Contrasting these methods, Stochastic Value Gradients (SVG) \cite{heess2015learning} re-evaluates rollouts with a learned model from off-policy data, accelerating learning through value gradients back-propagated through time via a learned model. In this work, we extend SVG to use imagined rollouts in latent spaces, accounting for model approximation errors via gradient averaging.

%\textbf{Models and Latent Representations:} With the advent of convolutional neural networks, there has been significant progress on learning image-based models and representations for planning and reinforcement learning \cite{ebert2018visual, cobra-dm, byravan2017se3}. 

There has also been work on combining latent space models and model-free RL. DeepMDP \cite{gelada2019deepmdp}, MERLIN \cite{wayne2018unsupervised}, CRAR \cite{franccois2018combined} and VPN \cite{oh2017value} combine representation learning with policy optimization via auxiliary losses such as observation reconstruction \cite{wayne2018unsupervised}, predicting the next latent state \cite{gelada2019deepmdp} or future values \cite{oh2017value}. Along these lines, we learn a latent representation that can be used for predicting (expected) future latent states, observations, rewards and values conditioned on the observed actions.

%\citep{ha2018recurrent} learns a latent space through a VAE, a recurrent world model to match the dynamics of the learned latent space and uses an evolutionary genetic algorithm to compute the actions to maximize expected reward in the latent space.

%\citep{silver2017predictron} proposes an end-to-end model learning and planning architecture that is trained completely based on value backups. Their $\lambda$-step preturn is somewhat similar to our averaging over N-step returns and they do rollouts and "planning" based on imagined states and the learned model.

%\citep{mbrl-atari} learns an environment model for atari through video prediction. This model is then used as a simulator for learning a policy through PPO. The model learning and policy learning steps are interleaved to generate better on-policy data towards the end. Overall, they are able to learn to play atari games well in about 200K iterations with the environment. They mention many possible future directions such as using the learned representations \& using model gradients which we do in this work.

%\citep{polo-uw} uses an MPC style planner with a global value function approximator to solve different tasks including in-hand manipulation. This is a bit similar to the idea of using CEM as the actor instead of an explicit policy representation for training.

%\cite{mb-mf-nagabandi} also does something similar where they first train a model based on random exploration, use CEM on the model to collect more data \& re-fit the model iteratively. They also propose a method to initialize a policy to fit the learned model-based controller followed by iterative improvement of the policy.

%\citep{gu-modelbasedacc, imagination-dm} propose different methods to integrate model-based "imagined" rollouts into model-free learning to improve sample efficiency.


%\citep{mve-feinberg} uses model-based imagined rollouts for improved value estimation similar to our k-step averaged returns for Q-learning. They do not use model gradients as in SVG and do not learn a state representation jointly. They also test on simple mujoco control environments (no pixels). Definitely worth a look though. 

%\citep{steve-nips19} extends this approach to use an ensemble of models, reward functions and horizons to interpolate the value estimates and show better performance than MVE.

%\citep{pmlr-v97-gelada19a} learns a model-based representation together with model-free RL for Atari tasks and show performance improvements. They use the reconstruction loss \& next-state prediction to condition the learned latent state. No transfer experiments are presented. This is similar to ours as they learn things together, no transfer though.

%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Transfer:}
One argument for model-based RL is the potential of transfer to tasks in the same environment. Sutton et al. \cite{sutton1990integrated} discuss early examples of this type of transfer on simple problems. Recently, Francois et al. \cite{franccois2018combined} showed encouraging results with a vision-based RL agent on 2D labyrinth tasks. Nagabandi et al. \cite{nagabandi2018learning, nagabandi2018deep} meta-learn predictive dynamics models to enable a model-based agent to rapidly adapt to changes in its environment. Other work on transfer in RL has focused on learning reusable skills e.g.\ in the form of embedding spaces \citep{hausman2018learning,florensa2017,dhruva2019}, successor representations \citep{barreto2017}, transferable priors \citep{galashov2018} or meta-policies \citep{finn2017,clavera2018}. As they learn ``behaviors'' rather than dynamics models, they are in a sense orthogonal and complementary to the ideas presented in this work.

